Fighting Fire with Light: A Case for Defending DDoS Attacks Using the Optical Layer

The DDoS attack landscape is growing at an unprecedented pace. Inspired by the recent advances in optical networking, we make a case for optical layer-aware DDoS defense (O-LAD) in this paper. Our approach leverages the optical layer to isolate attack traffic rapidly via dynamic reconfiguration of (backup) wavelengths using ROADMs---bridging the gap between (a) evolution of the DDoS attack landscape and (b) innovations in the optical layer (e.g., reconfigurable optics). We show that the physical separation of traffic profiles allows finer-grained handling of suspicious flows and offers better performance for benign traffic in the face of an attack. We present preliminary results modeling throughput and latency for legitimate flows while scaling the strength of attacks. We also identify a number of open problems for the security, optical, and systems communities: modeling diverse DDoS attacks (e.g., fixed vs. variable rate, detectable vs. undetectable), building a full-fledged defense system with optical advancements (e.g., OpenConfig), and optical layer-aware defenses for a broader class of attacks (e.g., network reconnaissance).

==> sections/definitions.tex <==
% \subsection{Definitions}
% \label{sec:definitions}

% % We formalize the terms necessary 
% To quantify the benefits of \name
% % % First, defining the graph structure of the AS, and then describing the classes of traffic that we consider. 
% we model the enterprise, where \name will be deployed, as a multi-graph $G = (V, E)$. In $G$, $V$ is a set of routers and switches. $E$ is a multi-set of ordered pairs, i.e., $E = \{(e,c)\}$. Let $e$ be an un-ordered pair of switches, $e = \{x, y\} : x,y \in V$, which represents a link (wavelength) between switches, and $c \in C$ be the capacity of the wavelength. $C = \{1, 10, 25, 40, 80, 100\}$ is the set of capacities available for wavelengths with today's commodity transceivers~\cite{fsdotcom}.

% \begin{figure}[htb!]
%     \center
%     \includegraphics[width=0.5\columnwidth]{figures/TrafficVennDiagram.jpg}
%     \caption{Classes of traffic flows ($F$) considered by \name. Attack traffic is shaded in red with diagonal hatches ($A$). Benign Traffic is shaded in solid blue. ($(S-A)\cup \neg S$).}
%     \label{fig:traffic_classes}
% \end{figure}

% In our model, flows ($F$) are denoted by a source and a destination address $(src, dst)$. We assume that the flows originate and terminate outside of $G$, and categorize them into four subsets. Flows can be Attack ($A$), Suspicious ($S$), Not Suspicious (or Trusted) ($\neg S$), and Benign ($B$). We use the terms: good, benign, and legitimate interchangeably when referring to non-attack traffic. However, $B$ traffic is not necessarily trusted traffic, $\neg S$. 

% The four classes are related as follows: All flows are either Suspicious or Trusted; $S \cup \neg S = F \And S \cap \neg S = \emptyset $. Attack traffic is a subset of Suspicious traffic; $A \subseteq S$. Trusted traffic is a subset of Benign traffic; $\neg S \subseteq B$. Benign traffic is $(S-A)\cup\neg S$. Figure~\ref{fig:traffic_classes} illustrates the different classes of traffic as a Venn-diagram.

==> sections/lab-based_experiments.tex <==
\section{Lab-based Experiments}
We will develop a lab-based experiment to demonstrate the performance benefit for good traffic in this setting using two Cisco 3560 switches and 100m of fiber. The lab testbed will consist of many hosts behind one switch and a scrubbing server running behind the other switch. The ingress switch identifies and transmits good traffic through the methodology presented in vFiber~\cite{vfiber}, allowing good traffic to traverse a physically distinct lambda from the suspicious traffic. We will show how to reduce a scrubber's load while providing better QoS for a client. 

We will measure the total latency for messages from a host to the server. We expect that as lambdas are allocated for $S$, we will detect a higher proportion of $\neg S$ flows, and the average latency for all legitimate flows ($\neg S \cup (S-A)$) will decrease over time as less trusted users' traffic is being scrubbed.

In a follow-up experiment, we will increase the scale of attacks while running \name, and show that we can provide mediation against attacks of grander scale as opposed to a solution which scrubs 100\% of ingress traffic. We will measure the volume of attack traffic required to severely degrade the value of the scrubbing service for a wavelength-diversion solution and standard solutions in which all traffic is scrubbed.


==> sections/latency_analysis.tex <==
% {\bf Latency Improvement:}
% Now, we consider three classes of traffic and reason about three improved latency for each of them with a reconfigurable lambda solution for direct DDoS attacks: Trusted Traffic, ($\neg S$), benign suspicious traffic ($S-A$), and their union, all good traffic ($(S-A)\cup \neg S$). What is the benefit for a client in terms of average latency for traffic during a DDoS attack when $\neg S$ traffic can traverse a physically distinct lambda, bypassing the scrubber? The total decrease in latency for trusted traffic is $\epsilon*T^{\neg S}$ seconds.  Similarly, the reduction of load at the scrubber is $T^{\neg S}$ Gbps.  We will vary the proportion of traffic that can be labeled $\neg S$ from 0 to 100 percent. The average latency, $\hat{L}$, for traffic to the client is a weighted average of the proportion of traffic that travels the scrubber, and the ratio of traffic that does not.

% \begin{equation}
%     \hat{L} = \frac{(\delta) T^{\neg S} + (\delta+\epsilon)T^{S}}{T}
% \end{equation}

% Where $\delta$ is the baseline delay through the network from ingress to $v$, and $\epsilon$ is the additional latency incurred at the scrubber. 

% %We plug a value for expected latency from origin routers $\delta = 100ms$. Let the time of additional latency $\epsilon = 50ms$, incurred by the scrubber. Figure~\ref{fig:latencyMode} illustrates the drop in latency for a client's good traffic when various proportions of the traffic can be directed directly to the client, and away from the scrubbing center.

% %\begin{figure}[]
% %    \center
% %    \includegraphics[width=0.98\columnwidth]{figures/latencyModel.png}
% %    \caption{The benefit for clients average latency is proportional to the amount of traffic that can be labeled as benign before scrubbing.}
% %    \label{fig:latencyMode}
% %\end{figure}

% {\bf Throughput improvement:}
% Now, consider the throughput that the network can forward to the client with FastPass and without FastPass. Recall that $T$ Gbps of ingress traffic is entering the system. Let $\hat{T}$ be the volume of traffic that we forward to the client. If we scrub 100\% of the ingress traffic, then the rate of traffic that we can forward to the client is limited by the bandwidth of the scrubbing appliances at the datacenter, $T^{D}$. However, if we can leverage re-configurable lambdas to send trusted traffic, $T^{\neg{S}}$ around the scrubbers, as in figure~\ref{fig:attack-model2}, then the total bandwidth to the client is augmented with the trusted traffic.

% \begin{equation}
%     \hat{T} = T^{D} + T^{\neg{S}}
% \end{equation}


% {\bf Significance of results:} The physical layer switching of $\neg S$ flows reduces the scrubber's load by an amount proportional to the capacity of good traffic. {\em \name} provides a benefit for the client, as she may receive $\neg S$ traffic with lower latency. Further, it gives an advantage to the AS administrators, as the reduced load at $d$ implies that they will be equipped to handle attacks of higher scales {\bf because good traffic can pass directly to the client}.



==> sections/related_work.tex <==
\section{Related Work}


Routing around congestion~\cite{smith2018routing, stone2000centertrack, van2006dynamic}

Reconfigurable optics  deployments~\cite{filer2016elastic, ghobadi2016optical, ghobadi2016projector, jin2016optimizing, singh2018radwan}

DDoS simulations for the US Fiber-optics backbone~\cite{kumar2017simulating}.

Technological enablers~\cite{openconfig, porter2013integrating}



==> sections/summary.tex <==
\section{Ongoing Work}

Table~\ref{tab:summary} summarizes the evaluation presented in section~\ref{sec:analysis}.

{\bf Note: I am still working on the indistinguishable v. distinguishable attack and fixed vs. variable rate attack types. It seems to make like any attack will be a linear combination of these three categories, so maybe I should consider them as such, i.e., direct distinguishable fixed rate attacks, direct distinguishable variable rate attacks, direct indistinguishable fixed rate attacks, direct indistinguishable variable rate attacks, etc...}

\begin{table}[htb!]
    \centering
    \begin{tabular}{c|c|c|c}
        \bf{Category}       & \bf{Spiffy}   & \bf{Scrubbing}& {\bf\name}  \\\hline
        \iffalse
        Distinguishable     & \checkmark    & \checkmark    & \checkmark \\
        Indistinguishable   & \checkmark    & \textendash   & \checkmark \\\hline
        Fixed-rate          & \checkmark    & \checkmark    & \checkmark \\
        Variable-rate       & \textendash   & \checkmark    & \checkmark \\\hline
        \fi
        Direct              & \textendash   & \checkmark    & \checkmark \\
        Indirect            & \checkmark    & \textendash   & \checkmark \\
        
        \end{tabular}
    \caption{Categories of DDoS attacks and coverage by various techniques.}
    \label{tab:summary}
\end{table}


